1-PAGER: One Pass Answer Generation and Evidence Retrieval

We present 1-Pager the first system that answers a question and retrieves evidence using a single Transformer-based model and decoding process. 1-Pager incrementally partitions the retrieval corpus using constrained decoding to select a document and answer string, and we show that this is competitive with comparable retrieve-and-read alternatives according to both retrieval and answer accuracy metrics. 1-Pager also outperforms the equivalent closed-book question answering model, by grounding predictions in an evidence corpus. While 1-Pager is not yet on-par with more expensive systems that read many more documents before generating an answer, we argue that it provides an important step toward attributed generation by folding retrieval into the sequence-to-sequence paradigm that is currently dominant in NLP. We also show that the search paths used to partition the corpus are easy to read and understand, paving a way forward for interpretable neural retrieval.

==> tables/tokenization.tex <==
\begin{table}[ht]
\begin{center}

% \begin{tabular}{c|c|c}
% \toprule
% Training sensitive & \multirow{2}{*}{Beam} & \multirow{2}{*}{EM} \\
% to tokenization &  & \\
% \midrule
% $\times$   & 1 & 26.4 \\
% $\checkmark$ & 1 & 28.7 \\
% \midrule
% $\times$ & 5 & 30.7 \\
% $\checkmark$ & 5 & 31.7 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{c|c}
\toprule
Rare Tokenization in training   & EM \\
\midrule
$\times$   & 26.4 \\
$\checkmark$ & 28.7 \\
% \midrule
% $\times$ & 5 & 30.7 \\
% $\checkmark$ & 5 & 31.7 \\
\bottomrule
\end{tabular}

\caption{Effect of appropriate tokenization in training}
\label{tab:tokenization}

\end{center}
\end{table}

==> tables/train_examples.tex <==
\begin{table*}[ht]
\begin{center}
\small
\begin{tabular}{p{0.9\textwidth}}
\toprule
 \textbf{Generated Search Paths}  \\
\midrule
Q: when does guardian of the galaxy come out\\ SP: Guardians of the Galaxy (film) >> premiered in Hollywood >> August 1, 2014\\ \midrule
Q: when did the us get involved with puerto rico\\ SP:  History of Puerto Rico >> Spanish–American War, Puerto >> 1898\\ \midrule
Q: what is the stripes on the american flag mean\\ SP:  Flag of the United States >> 13 stripes >> thirteen British colonies\\ \midrule
Q: when did martial law ended in the philippines\\ SP:  Proclamation No. 1081 >> President Marcos >> 17 January 1981\\ \midrule
Q: who created the quote keep calm and carry on\\ SP:  Keep Calm and Carry On >> produced by the British government  >> British government\\ 
\bottomrule
\end{tabular}

\caption{Example queries and search paths from training. Last keyword is the answer.}
\label{tab:train_examples}

\end{center}
\end{table*}

==> tex/future_work.tex <==
\section{Future Work}
- Greedy decoding beam lacks diversity. Small temperature may help in exploration.

